Fast-Response Variable Frequency DC-DC Converters Using Switching Cycle Event-Driven Digital Control

This paper investigates a new method to model and control variable-frequency power converters in a switching-synchronized sampled-state space for cycle-by-cycle digital control. There are a number of significant benefits in comparison to other methods including fast dynamic performance together with ease of design and implementation. Theoretical results are presented and verified through hardware, and simulations of a current-mode buck converter with constant on-time and a current-mode boost converter with constant off-time. Dynamic voltage scaling for microprocessors and LiDAR are among the applications that can benefit.

==> text.tex <==
\begin{align}
    a_1 =\,&
    1-2(\hat{\tau}_1^{-1}+\hat{\tau}_3^{-1})-\frac{\lambda^2+(1-\lambda)^2}{2}\hat{\tau}_1^{-1} \hat{\tau}_2^{-1},  \\
    d_1 =\,& ( \lambda \hat{\tau}_1^{-1} + \frac{\lambda^2}{2}\hat{\tau}_1^{-1} \hat{\tau}_2^{-1} - 1)(\hat{\tau}_1^{-1} + \hat{\tau}_3^{-1}) \nonumber \\
    & -\left(1+(1-\lambda)\hat{\tau}_1^{-1} -2(\hat{\tau}_1^{-1}+\hat{\tau}_3^{-1}) - \frac{\lambda^2}{2}\hat{\tau}_1^{-1}\hat{\tau}_2^{-1} \right) \nonumber \\
    &\times (1-\lambda)\hat{\tau}_1^{-1} \hat{\tau}_2^{-1},  \\
    d_2 =\,& \left(\lambda \hat{\tau}_1^{-1} +\frac{\lambda^2}{2}\hat{\tau}_1^{-1} \hat{\tau}_2^{-1}-1\right)(\hat{\tau}_1^{-1} + \hat{\tau}_3^{-1}) + \lambda \hat{\tau}_1^{-1} \hat{\tau}_2^{-1}, \\
    g_1 =\,& \left(\lambda \hat{\tau}_1^{-1} - \left(1 - \lambda \hat{\tau}_1^{-1} - \frac{\lambda^2}{2} \hat{\tau}_1^{-1} \hat{\tau}_2^{-1}\right)\frac{\hat{\tau}_1^{-1}+\hat{\tau}_3^{-1}}{\hat{\tau}_2^{-1}}\right)R, \\
    b_1 =\,& \frac{d_1}{d_2}.
\end{align}
